MOSEL: Inference Serving Using Dynamic Modality Selection

Rapid advancements over the years have helped machine learning models reach previously hard-to-achieve goals, sometimes even exceeding human capabilities. However, to attain the desired accuracy, the model sizes and in turn their computational requirements have increased drastically. Thus, serving predictions from these models to meet any target latency and cost requirements of applications remains a key challenge, despite recent work in building inference-serving systems as well as algorithmic approaches that dynamically adapt models based on inputs. In this paper, we introduce a form of dynamism, modality selection, where we adaptively choose modalities from inference inputs while maintaining the model quality. We introduce MOSEL, an automated inference serving system for multi-modal ML models that carefully picks input modalities per request based on user-defined performance and accuracy requirements. MOSEL exploits modality configurations extensively, improving system throughput by 3.6$\times$ with an accuracy guarantee and shortening job completion times by 11$\times$.

==> sections/algorithm.tex <==
\section{Optimize Dropping Policies}

There are various ways to deploy a model in production environments. Examples
include multi-stream~\cite{?}, MiG instances~\cite{?}, distributed~\cite{?},
time sharing~\cite{?}. It's challenging to estimate model performance under
these varying environments. Therefore, An exploration module proposes new
modality dropping policies to run on the hardware. The run time statistics are
recorded. We discuss module design choices in the following subsections.

We propose a machine learning (ML)-based framework to solve this problem. 

\textbf{Initialization}

\textbf{Score}

\textbf{Crossover}

\textbf{Mutation}

\subsection{Exploration Stage}

!!!!!!
splitting a batch into several micro-batches happens right before inference stage.
There are potentially many places modality drop can happen.
more specifically, we say which part of a system may benefit from dropping.

1. network transport: intuitive, reducing data transferred naturally reduces transmission latency
    - better handle for bursty traffic?
    - what to squeeze out from network?
2. not splitting into micro-batches, but use each modality as is. For example, 
we can reorganize multple requests into uniform batch shape: 32: audio, then 32 video
then 32 both. We fill them up and then perform inferences individually, ensuring
in the long run average latency is guaranteed.
    - we just profiler modality-specific accuracy, then dynamically choose which
    option to use, as long as long time avg accuracy is met.
3. what we do right now: split batch into microbatches
    - we can keep rnunning this algorithm offline and constantly update the policy!!
        - scheduling between inf and profiling!
    - we analyse why certain model benefit from it
    - obvisouly, our GA algo will need take less focus
    - dynamicaly choose fill up SLO slot.
    - we can even drop data during inference! as long as fusion didn't happen!!!
4. for small batch (1), we use easier data to inf, which will leave additional space
for more accurate inferences. We can dynamically add/reduce accuracy, as long as
avg acc and SLO is guaranteed
5. graph recombine? 
6. modality? dynamic fusion?
7. gating layer, but also take latency into account (training parameter)
    - gating : lat
      yes : no
      yes : yes
      no : yes
      no : no
    - on even a higher level, we take system metrics into routing/model layers and routing
    then accordingly. this applies to all dynamic NN.
    - should model itself handle the accuracy vs latency/performance tradeoff?
    - ENVIRONMENT-AWARE AI!!
        - first question: will dynamic nn behave differently in the presence of environment varibales?
8. we sell modality as METERICS?
    - NOT ALL MODALITIES ARE EQUAL!
        - Given that statement, what can we do?
            - drop modality
            - ??
    - not all modalities are important!
    - use case 1: we can use metrics to drop modality
    - other optimization: quantization, etc.
9. like INFaaS, we have a large navigation space: not only modality drop policy
, but also reorder query submission, stream vs sequential submission vs MIG, etc.
    - we have MODEL-VARIANT, can we have DATA-VARIANT?
        - With LLM, can we choose which data is more suitable for the job? e.g. rgb, vs flow vs greyscale, etc..
            - capacity factor in MoE model, batch-priority routing drop
            - text -to -speech first?
        - task-specific optimization! wwhereas model-variant is not task-specific
        - skip audio/video frames?
        - partially dropped data
        - scaled-down images
        - low-quality audios, reduce phoneme number
        - text?
        - different format of images have different system implications
        - use raw documennt or involved OCR?


==> sections/introduction.tex <==
\section{Introduction}

% \note{\bf Briefly explain multi modal DNN serving}
Machine Learning (ML) models have become increasingly more important in various real-world applications such as object recognition~\cite{wang2023yolov7, dosovitskiy2020image}, video understanding~\cite{kazakos2019TBN, arnab2021vivit}, speech recognition~\cite{yuhas1989integration, chen1998audio, shi2021learning}, natural
language processing~\cite{brown2020language, devlin2018bert}, visual question answering~\cite{yu2017multi}, and many more. Multimodal learning~\cite{yuhas1989integration, ngiam2011multimodal} is an emerging technique combining data of different modalities to provide prediction cooperatively, enhancing ML models' prediction accuracy.  
%preventing information loss from data of one modality. 
%Multimodal learning has been proved to improve prediction performance of many tasks, including X~\cite{}, Y~\cite{} and Z~\cite{}.


\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/motivation-sketch.jpeg}
    \caption{\it Comparison of different modalities for different multi-modality models. We compare different models and their input modalities' (i) contribution to the result accuracies, (ii) processing latencies and (iii) resource (i.e., memory) consumption. \bd{Figure 2?}}
    \label{fig:modality-contribution}
\end{figure}

% Typically, the development of a ML model involved two distinct stages: training and inference.
% Training stage tend to be resource-intensive, and less sensitive to end-to-end latency. In contrast,
In a typical multimodal model, data of different modalities contribute differently to the result of prediction, while also consuming varying computational resources and contributing differently to the end-to-end prediction latency. As described in greater detail in Section~\ref{sec:observation}, we empirically find that % how data of different modalities contribute to prediction accuracy, as well as processing time and resource consumption associate with each modality. We could observe that 
some modalities (e.g., \aditya{fill} ) contribute significantly to prediction accuracy while not being the major contributor to resource use and processing time, while other modalities (e.g., \aditya{fill}) consume a significant amount of resources while only marginally contributing to prediction accuracy. 

These examples raise interesting questions for inference using multimodal ML models. Prior work has shown that inference workloads dominate ML infrastructure costs~\cite{?}, and such workloads have become key targets for improving both resource efficiency and latency. Furthermore,  
%The inference applications are both resource and latency sensitive~\cite{?}, and 
the interactive nature of inference tasks means inference systems
should be able to handle dynamic workloads without violating user- (e.g., end-to-end latency) or resource-constraints (e.g., available device memory). For multimodal ML models, the varying accuracy benefits and latency costs introduced by processing different modalities of data unveil exciting opportunities for inference systems to explore ways to \textit{dynamically} reason about relationships among latency targets and resource usages processing data of different modalities. This implies that for multi-modality ML models, input data of different modalities imply different \textit{data efficiencies}: 
%\lx{<- This is not connecting -- is resource efficiency part of the optimization or are we just saying that we are only using limited resources and resource inefficiencies will reflect on the performance degradation?}

In a latency-sensitive deployment scenario such as action recognition from wearable devices~\cite{kazakos2019TBN}, multi-modality input data (e.g., RGB, audio, flow) is decoded and sent to server runtime for real-time analysis of action~\cite{related work for offload}. While the entire recognition process has an end-to-end latency requirement~\cite{find reasonable latency requirement}, the ``latency budget'' for each request to be processed at the inference runtime could constantly change due to unpredictable environmental factors such as unexpected network delays. 
% Serving inference requests with dynamic requirements in real-time has been explored extensively in the past~\cite{}. 
Comparing to single-modal inference, multimodal models have provided a new perspectives exploring tradeoff between prediction quality and user requirement. For example, a temporal binding network (TBN) combines RGB (from video), optical flow (from video) and log spectrogram (from audio) to provide action recognition. For a user who demand expected prediction accuracy of action recognition (e.g. verb prediction) of 75\%, the model needs to process all modality input to achieve target accuracy while resulting in an inference latency of 516ms. Alternatively, if the user relax the accuracy demand by 5\% (to 70\%), the model could selectively processes ``key modalities'' (e.g., optical flow and spectrogram only) and complete the inference process in 358ms, which effectively prevents degrading user experience in the scenario where unexpected delays occur. 

In this paper, we focus on a typical deployment scenarios for multi-modal DNN inference~\cite{li2021low}: a model serving runtime processes inference requests composed by data of varying modalities, arriving at unpredictable pattern~\cite{}. These requests are generated by users with different expectation on model performance (e.g., prediction accuracy). 
Additionally, users of these models may impose \emph{environmental constraints} including service-level objectives (SLOs) such as end-to-end latency, processing throughput and constraints on available device memory and energy consumption. 
%\lx{<- This is duplicated from the previous section. You could remove this entirely?}

% For example, AR. When a user wants to ask the device to identify an object.
% The video would then be transferred to the server side, which would perform
% inference and return the result~\cite{}. The transmission process are vulnerable to many
% environmental variables, such as network congestion. Such interferences could
% change latency constraint of the inference task when request is received. 

% use a very specific example, , if audio, video, and audio+video has
% accuracy: 66%, 72% 74%. Given batch size 64, if a user want the inference task
% to finish under 10 ms, then only selecting audio would meet the requirement;
% if the user wants high accuracy, then he/she needs to select both video and audio
% to meet the accuracy objectives. If the user wants to 72%, there are many modality
% selection plans that can meet the accuracy objectives.

It's common in production settings to witness bursty queries, which leads to
immense pressure to complete these tasks in a timely fashion. Compromising data
quality can reduce the computational resource required, therefore mitigating
the system load.\lx{<- suggest to remove}


% 1. different users/tasks require has different resource/accuracy requirement.

% 2. Outside factor (e.g. transmission delay, network congestion, etc..) could
% affect the e2e latency, thus requiring inference latency to be adjusted to accomodate
% the delay.

% With changing inference latency requirements, we can selectively process
% modalities to accomodate inference efficiency.


% Traditional inference systems are model-agnostic.
Multi-modality models provide unique opportunities for the inference systems to be able to reason about the selection of deployment configurations that achieve the balance between achieving prediction accuracy goal while also satisfying environmental constraints. 
Traditional inference frameworks~\cite{} typically explore such tradeoff space by exploring options to degrade model qualities, but unable to reason about data efficiencies among input data.
\lx{In this work, we exploit...}
% Could we using dropping so that some queries that won't be able to run due to SLO violation be available?
